High-Accuracy Low-Precision Training

Low-precision computation is often used to lower the time and energy cost of machine learning, and recently hardware accelerators have been developed to support it. Still, it has been used primarily for inference - not training. Previous low-precision training algorithms suffered from a fundamental tradeoff: as the number of bits of precision is lowered, quantization noise is added to the model, which limits statistical accuracy. To address this issue, we describe a simple low-precision stochastic gradient descent variant called HALP. HALP converges at the same theoretical rate as full-precision algorithms despite the noise introduced by using low precision throughout execution. The key idea is to use SVRG to reduce gradient variance, and to combine this with a novel technique called bit centering to reduce quantization error. We show that on the CPU, HALP can run up to $4 \times$ faster than full-precision SVRG and can match its convergence trajectory. We implemented HALP in TensorQuant, and show that it exceeds the validation performance of plain low-precision SGD on two deep learning tasks.

==> deep.tex <==
\section{Applications to Deep Learning}
\label{sec:deep}
\begin{figure}
\centering
\begin{tabular}{c c}
	\includegraphics[width=0.475\linewidth]{figures/charrnn_train_loss.pdf}	&
	\includegraphics[width=0.475\linewidth]{figures/cifar_train_loss.pdf} \\
	\includegraphics[width=0.475\linewidth]{figures/charrnn_val_acc.pdf}	&
	\includegraphics[width=0.475\linewidth]{figures/cifar_val_acc.pdf}
\end{tabular}
\caption{Training loss and validation perplexity on LSTM for character level language modeling on TinyShakespeare dataset (Left). Training loss and Validation accuracy on ResNet for image recognition on CIFAR10 dataset.}
\label{fig:dl_results}
\end{figure}

In this section, we empirically evaluate LP-SVRG on both convolutional neural networks (CNN) and recurrent neural networks (RNN). We conduct CNN experiment using a ResNet~\cite{he2016deep} with 3 basic ResNet building blocks on CIFAR10~\cite{krizhevsky2014cifar} for image recognition. The 3 ResNet blocks use $16, 32, 64$ channels of $3\times3$ kernels respectively. It has 7 convolutional layers and 1 fully connected layer. For the RNN experiment, we evaluate LP-SVRG on the character language modeling with TinyShakespeare dataset~\cite{karpathy2015visualizing}. The RNN model consists of 2 LSTM layers, each with 128 hidden units. We set learning rate to 0.5 and 1.0 uniformly in the CNN experiments and in the RNN experiments respectively. We use the above protocol to validate two claims 1) when using 16 bit fixed point model representation, LP-SVRG can reach task-specific solution matching the quality of full precision SVRG, 2) in fixed point low precision setting, LP-SVRG can outperform low precision SGD by reducing gradient variance. 

In Figure~\ref{fig:dl_results}, on both the LSTM and ResNet model, we observe that 16 bit LP-SVRG can closely match the full precision SVRG on training loss and validation metrics. Specifically on the LSTM model, the validation perplexity from full precision SVRG starts to increase after 60 epochs due to overfitting. On the other hand, the 16 bit SVRG still keeps an stable validation perplexity, possibly as a result of the fact that low precision representation can help reduce overfitting. 


The comparison between LP-SVRG and low precision SGD (using the same fixed representation as with LP-SVRG) also reveals the benefits of variance reduction in low precision training. More specifically, LP-SVRG demonstrate a validation perplexity improve of 0.06 over SGD in 16 bit training. This benefit is even more noticeable in the 8 bit training with an validation perplexity improvement of 0.23. On ResNet model, LP-SVRG shows improved validation accuracy of 0.7 and 1.9 respectively in 16 bit and 8 bit low precision training. These observations validates the benefits of gradient variance reduction in low precision training.


